Efficient Data Shapley for Weighted Nearest Neighbor Algorithms

This work aims to address an open problem in data valuation literature concerning the efficient computation of Data Shapley for weighted $K$ nearest neighbor algorithm (WKNN-Shapley). By considering the accuracy of hard-label KNN with discretized weights as the utility function, we reframe the computation of WKNN-Shapley into a counting problem and introduce a quadratic-time algorithm, presenting a notable improvement from $O(N^K)$, the best result from existing literature. We develop a deterministic approximation algorithm that further improves computational efficiency while maintaining the key fairness properties of the Shapley value. Through extensive experiments, we demonstrate WKNN-Shapley's computational efficiency and its superior performance in discerning data quality compared to its unweighted counterpart.

==> checklist.tex <==
\section*{Checklist}


% % %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references. For each question, choose your answer from the three possible options: Yes, No, Not Applicable.  You are encouraged to include a justification to your answer, either by referencing the appropriate section of your paper or providing a brief inline description (1-2 sentences). 
% Please do not modify the questions.  Note that the Checklist section does not count towards the page limit. Not including the checklist in the first submission won't result in desk rejection, although in such case we will ask you to upload it during the author response period and include it in camera ready (if accepted).

% \textbf{In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.}
% % %%% END INSTRUCTIONS %%%


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. Yes, see Section \ref{sec:shapley-for-binary}. 
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. Yes, see Section \ref{sec:shapley-for-binary}.
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. Yes. 
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. Yes. 
   \item Complete proofs of all theoretical results. Yes. 
   \item Clear explanations of any assumptions. Yes.    
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). Yes.
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). Yes. 
    \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). Yes.
    \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). Yes.
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. Yes.
   \item The license information of the assets, if applicable. Yes.
   \item New assets either in the supplemental material or as a URL, if applicable. Not Applicable.
   \item Information about consent from data providers/curators. Not Applicable.
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. Not Applicable.
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. Not Applicable.
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. Not Applicable.
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. Not Applicable.
 \end{enumerate}

 \end{enumerate}


==> newpseudocode.tex <==
\centerline{
\scalebox{0.75}{
\begin{minipage}[t]{1\linewidth}
\begin{algorithm}[H]
\caption{Weighted KNN-Shapley for binary classification}
\label{alg:efficient-wknn}
\begin{algorithmic}[1]
\Procedure{WeightedKNNShapley}{}

\State

\For{$i = 1$ to $N$}

\State Initialize $\Fi[m, \ell, s] = 0$ for $m = 1, \ldots, N, \ell=1, \ldots, N, s \in V$. 

\For{$m = 1$ to $N$, $m \ne i$}
\State $\Fi[m, 1, w_m] = 1$
\EndFor

\State

\For{$\ell = 2$ to $K-1$}
\State $F_0[:] = \sum_{t=1}^{\ell-1} \Fi[t, \ell-1, :]$
\For{$m = \ell$ to $N$}
\For{$s \in V$}
\State $\Fi[m, \ell, s] = F_0[s - w_m]$
\EndFor
\EndFor
\EndFor

\State 

\For{$\ell = 2$ to $K-1$}
\For{$m = \ell$ to $N$}
\For{$s \in V$}
\State $\Fi[m, \ell, s]
= \sum_{t=1}^{m-1} \Fi[t, \ell-1, s - w_m]$
\EndFor
\EndFor
\EndFor

\State

\For{$s \in V$}
\State 
$R_0[s] = \sum_{t=1, t \ne i}^{ \max(i+1, K+1)-1 } \Fi[t, K-1, s]$. 
\EndFor

\For{$m = \max(i+1, K+1)$ to $N$}
\State 
$\Ri[m] = \sum_{s \in [-w_i, -w_m)} R_0[s]$. 
\State $R_0 = R_0 + \Fi(m, K-1, :)$. 
\EndFor

\State

\State $G_i(0) = 0$. \Comment{For fair} 

\State

\For{$\ell = 1$ to $K-1$}
\State
$\Gil = \sum_{m \in [N] \setminus i} \sum_{s \in [-w_i, 0)} \Fi\left[m, \ell, s\right]
$. 
\EndFor

\State 

\State $\phi_i = \frac{1}{N} \sum_{\ell=0}^{K-1} \frac{\Gil}{{N-1 \choose \ell}} + \sum_{m = \max(i+1, K+1)}^N \Ri[m] {m-1 \choose K}^{-1} \frac{1}{m}
$. 

\EndFor

\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{minipage}
}
}

==> oldpseudocode.tex <==
\centerline{
\scalebox{0.75}{
\begin{minipage}[t]{1\linewidth}
\begin{algorithm}[H]
\caption{Weighted KNN-Shapley for binary classification ($O(N^2)$ runtime)}
\label{alg:efficient-wknn}
\begin{algorithmic}[1]
\Procedure{EfficientWeightedKNNShapley}{}

\State Initialize $F(m, \ell, s) = 0$ for $m = 1, \ldots, N, \ell=1, \ldots, N, s \in V$. 

\State

\For{$m = 1$ to $N$}
\State $F(m, 1, w_m) = 1$
\EndFor

\State

\For{$\ell = 2$ to $K-1$}
\For{$m = \ell$ to $N$}
\For{$s \in V$}
\State $F(m, \ell, s)
= \sum_{t=1}^{m-1} F(t, \ell-1, s - w_m)$
\EndFor
\EndFor
\EndFor

% \State 

% \For{$\ell = K$ to $N$}
% \For{$m = K$ to $N$}
% \For{$s \in V$}
% \State $F(m, \ell, s) = \sum_{t=1}^{m-1} F(t, K-1, s) \cdot {N-m \choose \ell-K}$
% \EndFor
% \EndFor
% \EndFor

\State

\For{$i = 1$ to $N$}

\For{$m = 1$ to $N$, $m \ne i$}
\State $\Fi(m, 1, w_m) = 1$
\EndFor

\State

\For{$\ell = 2$ to $K-1$}
\For{$m = \ell$ to $N$, $m \ne i$}
\For{$s \in V$}
\State $\Fi\left[m, \ell, s\right] = 
\begin{cases}
F(m, \ell, s) - \Fi(m, \ell-1, s-w_i) & i < m \\
F(m, \ell, s) & i > m
\end{cases}
$
\EndFor
\EndFor
\EndFor

% \State

% \For{$\ell = K$ to $N-1$}
% \For{$m = \max(i+1, K-1)$ to $N$}
% \For{$s \in V$}
% \State $\Fi\left[m, \ell, s\right] = 
% \begin{cases}
% F(m, \ell, s) - \Fi(m, \ell-1, s-w_i+w_m) \cdot {N-m \choose \ell-K} & i < m \\
% 0 & i > m
% \end{cases}
% $
% \EndFor
% \EndFor
% \EndFor

\State

\For{$s \in V$}
\State 
$R_0[s] = \sum_{t=1, t \ne i}^{ \max(i+1, K+1)-1 } \Fi[t, K-1, s]$. 
\EndFor

\For{$m = \max(i+1, K+1)$ to $N$}
\State 
$\Ri[m] = \sum_{s \in [-w_i, -w_m)} R_0[s]$. 
\State $R_0 = R_0 + \Fi(m, K-1, :)$. 
\EndFor

\State

\State $G_i(0) = 0$. \Comment{For fair} 

\State

\For{$\ell = 1$ to $K-1$}
\State
$\Gil = \sum_{m \in [N] \setminus i} \sum_{s \in [-w_i, 0)} \Fi\left[m, \ell, s\right]
$. 
\EndFor

\State 

\State $\phi_i = \frac{1}{N} \sum_{\ell=0}^{K-1} \frac{\Gil}{{N-1 \choose \ell}} + \sum_{m = \max(i+1, K+1)}^N \Ri[m] {m-1 \choose K}^{-1} \frac{1}{m}
$. 

\EndFor

\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{minipage}
}
}



==> pseudocode-multiclass.tex <==
\centerline{
\scalebox{0.8}{
\begin{minipage}[t]{1\linewidth}
\begin{algorithm}[H]
\ifinappendix
    \caption{Weighted KNN-Shapley for multiclass classification (Runtime-optimized version)}
    \label{alg:efficient-wknn-multiclass}
\else
    \caption{Weighted KNN-Shapley for multiclass classification (reader-friendly version)}
    \label{alg:efficient-wknn-readable-multiclass}
\fi
\begin{algorithmic}[1]

\State \textbf{Input:} 
\begin{itemize}
    \item $K$ -- hyperparameter of weighted KNN algorithm. 
    \item $\zval = (\xval, \yval)$ -- the validation point. 
    \item $D = \{z_i = (x_i, y_i)\}_{i=1}^N$ -- sorted training set where $d(x_i, \xval) \le d(x_j, \xval)$ for any $i \le j$.
    \item $\mstar$ -- hyperparameter for SV approximation (Section \ref{sec:deterministic-approx}). 
    $\mstar = N$ for exact SV calculation. 
\end{itemize}

\State

\State Compute the weight $w_i = \weightfunc(x_i)$ for $i \in \{1, \ldots, N\}$. 

\State

\For{$i \in \{1, \ldots, N\}$}

\State

\State \cmt{Initialize $\Fi$}
\State Initialize $\Fi[m, \ell, \s] = 0$ for $m \in \{1, \ldots, \mstar \}, \ell \in \{1, \ldots, K-1\}, \s \in \wspace^C$. 

\For{$m \in \{ 1, \ldots, \mstar \} \setminus \{i\}$}
\State $\Fi[m, 1, w_m \e_{y_m}] = 1$
\EndFor

\State 

\ifinappendix
    \State \cmt{Compute $\Fi$ \textcolor{blue}{(Runtime-optimized version)}}
    \For{$\ell \in \{2, \ldots, K-1\}$}
    \State $F_0[:] = \sum_{t=1}^{\ell-1} \Fi[t, \ell-1, :]$
    \For{$m \in \{ \ell, \ldots, \mstar \} \setminus \{i\}$}
    \For{$\s \in \wspace^C$}
    \State $\Fi[m, \ell, \s] = F_0[\s - w_m \e_{y_m} ]$
    \EndFor
    \EndFor
    \EndFor
\else
    \State \cmt{Compute $\Fi$ \textcolor{blue}{(Runtime-optimized version in Appendix \ref{appendix:pseudocode})}}
    
    \For{$\ell \in \{2, \ldots, K-1\}$}
    \For{$m \in \{ \ell, \ldots, \mstar \} \setminus \{i\}$}
    \For{$\s \in \wspace^C$}
    \State $\Fi[m, \ell, \s]
    = \sum_{t=1}^{m-1} \Fi[t, \ell-1, \s - w_m \e_{y_m}]$
    \EndFor
    \EndFor
    \EndFor
\fi

\State

\ifinappendix
    \State \cmt{Compute $\Rim$ \textcolor{blue}{(Runtime-optimized version)}}
    \For{$\s \in \wspace^C$}
    \State 
    $R_0[s] = \sum_{t=1, t \ne i}^{ \max(i+1, K+1)-1 } \Fi[t, K-1, s]$. 
    \EndFor
    \For{$m \in \{ \max(i+1, K+1), \ldots, \mstar \}$}
    \State 
    $\Rim = 
    \begin{cases}
    \sum_{t=1}^{m-1} \sum_{s \in [-\wtil_i, -w_m \e_{y_m})} R_0[s] & \text{for } y_i = \yval \\
    \sum_{t=1}^{m-1} \sum_{s \in [-w_m \e_{y_m}, -\wtil_i)} R_0[s] & \text{for } y_i \ne \yval 
    \end{cases}
    $
    \State $R_0 = R_0 + \Fi[m, K-1, :]$
    \EndFor
\else
    \State \cmt{Compute $\Rim$ \textcolor{blue}{(Runtime-optimized version in Appendix \ref{appendix:pseudocode})}}
    
    \For{$m \in \{ \max(i+1, K+1), \ldots, \mstar \}$}
    \State 
    $\Rim = \sum_{t=1}^{m-1} \sum_{\s \in \mS_{i, m}} \Fi[t, K-1, \s]$. 
    \EndFor
\fi

\State

\State \cmt{Compute $\Gil$}

\State $\Gizero = \ind[w_i < 0]$.\footnote{Recall that we define $\U(S) = \ind \left[ \sum_{j=1}^{\min(K, |S|)} \widetilde{w}_{(j)} \ge 0 \right]$, hence $\U(\{z_i\}) - \U(\emptyset) \in \{-1, 0\}$ and is equal to $-1$ if and only if $w_i < 0$.}

\For{$\ell \in \{1, \ldots, K-1\}$}
\State
$\Gil = \sum_{t=1}^{m-1} \sum_{\s \in \mS_{i}} \Fi\left[m, \ell, \s\right]$. 
\EndFor

\State 

\State \cmt{Compute the Shapley value for $z_i$}

\State $\phi_{z_i} = \sign(w_i) \left[
\frac{1}{N} \sum_{\ell=0}^{K-1} \frac{\Gil}{{N-1 \choose \ell}} + 
\sum_{m = \max(i+1, K+1)}^{\mstar} \frac{\Rim}{ m {m-1 \choose K} } 
\right]$.\footnote{
$\sign(w) = 
\begin{cases}
    1 & w>0 \\
    0 & w=0 \\
    -1 & w<0    
\end{cases}$.
} 

\EndFor
\end{algorithmic}
\end{algorithm}
\end{minipage}
}
}

==> sec_multiclass_extension.tex <==
\subsection{Naive Extension from Binary Classification Setting}
\label{sec:multi-class-exact}

% In order to extend our algorithm to compute the Data Shapley for multi-class KNN classifiers, we refine our approach to move beyond the simplicity of the binary setting. 

We first discuss a simple, direct extension of our exact WKNN-Shapley algorithm from binary to multi-class classification setting. 
In Algorithm \ref{alg:efficient-wknn-readable}, the main idea is to maintain a record of $\Fi[m, \ell, s]$ for a singular scalar value $s$ which represents the summation of ``signed weights'' $\wtil_j$. In order to extend this approach to the multi-class setting, it is natural to enhance this scalar representation to a ``histogram'' depiction, $\Fi[m, \ell, \s]$, where $\s$ is the vector sum of weights for each data point, and the weights are in the form of one-hot encoding. 
That is, in the multi-class setting, $\Fi$ is augmented to record the number of subsets such that the sum of weights of the data points in the one-hot encoding is equal to the histogram $\s$ (subject to the conditions analog to those in Definition \ref{def:Fi-binary}). 
While this direct extension can compute the exact Data Shapley for the utility function in (\ref{eq:util}), it has a time complexity of $O(K^{1+C} N^2 \nwspace^C)$ as we need to record $\Fi[m, \ell, \s]$ for all possible histograms $\s \in \wspace_{(K)}^C$. 
This is manageable for datasets with a modest size of class space. However, for datasets with a large class space, this complexity can render the runtime prohibitively large. 

% Fortunately, the recursive relationships for the multi-class $\Fi$ are similar to those from the binary setting. 
% We defer the full algorithm for the multi-class setting in Appendix \ref{appendix:multiclass}.


\subsection{Utility Function that Enables More Efficient Computation of WKNN-Shapley}
\label{sec:multiclass-heuristic}

Due to the above-mentioned computational bottleneck, we introduce an alternative utility function for weighted KNN classifiers, which not only reflects the KNN classifiers' performance but also paves the way for a more efficient Data Shapley computation analogous to that of the binary setting.

% While the algorithm from the previous section gives the procedure for computing the exact Data Shapley for WKNN multiclass classifier, its time complexity is $O(K N^2 \nwspace^C)$. While this might be acceptable for the classification task where the number of classes is relatively small, the runtime could be prohibitive when the number of classes is large. Hence, in this section, we propose a simple alternative of the utility function for weighted multiclass classification which induces a much more efficient way to compute Data Shapley.

\textbf{Alternative Utility Function for Weighted Hard-Label KNN Classifiers.} 
% Recall that the utility function of hard-label KNN can be written as 
% $
% \U(S; \zval) =
% \ind \left[ \yval \in \argmax_{ c \in \C } \sum_{j=1}^{\min(K, |S|)} w_{\alpha_{\xval}^{(S, j)}} \ind[y_{\alpha_{\xval}^{(S, j)}} = c] \right]
% $. 
For a class $c \ne \yval$, we denote 
% \begin{align}
% \U^{(c)}(S; \zval) 
% :=
% \ind\left[ 
% \sum_{j=1}^{\min(K, |S|)} w_{\alpha_{\xval}^{(S, j)}} \ind[y_{\alpha_{\xval}^{(S, j)}} = \yval] 
% \ge 
% \sum_{j=1}^{\min(K, |S|)} w_{\alpha_{\xval}^{(S, j)}} \ind[y_{\alpha_{\xval}^{(S, j)}} = c]
% \right]
% \end{align}
% \tianhao{After correction}
\begin{align}
\U^{(c)}(S; \zval) 
:=
&\ind\left[ 
\sum_{j=1}^{\min(K, |S^{(c)}|)} w_{\alpha_{\xval}^{(S^{(c)}, j)}} \ind[y_{\alpha_{\xval}^{(S^{(c)}, j)}} = \yval] 
\right. \nonumber \\
&\left.~~~\ge \sum_{j=1}^{\min(K, |S^{(c)}|)} w_{\alpha_{\xval}^{(S^{(c)}, j)}} \ind[y_{\alpha_{\xval}^{(S^{(c)}, j)}} = c]
\right]
\end{align}
where 
$
S^{(c)} 
:= \{(x, y) \in S: y \in \{\yval, c\} \}
$ is the subset of $S$ whose labels are either $\yval$ and $c$, and we propose an alternative utility function as follows:
\begin{align}
\Ualter(S; \zval) 
:= 
\frac{1}{C-1}
\sum_{c \in [C] \setminus \yval} 
\U^{(c)}(S^{(c)}; \zval)
\label{eq:util-multiclass}
\end{align}
Note that for binary classifiers, the new utility function $\Ualter$ reduces to the original $\U$. 
\textbf{Interpretation of the Alternative Utility Function:} 
The alternative utility function, $\Ualter$, captures a fine-grained view of the classifier's performance. Instead of just deciding based on whether a prediction is correct as the original utility function in (\ref{eq:util}), it assesses the \emph{rank} of the prediction confidence for the correct class, $\yval$, among all potential class predictions in the weighted KNN classifier. 
% For instance, if the queried example $\xval$ is correctly being classified, then $\Ualter(S; \zval) = 1$ which means classes $\yval$ receive the highest amount of weighted voting by the training points. 
Hence, $\Ualter$ provides insight into not just the correctness, but also the relative confidence of a prediction with respect to other classes. 
\tianhao{This interpretation is not very precise; polish the writing}

\textbf{Data Shapley for $\Ualter$.}
The linearity axiom of the Shapley value provides that 
\begin{align*}
\phi_{z_i}( \Ualter ) = 
\frac{1}{C-1} \sum_{c \in [C] \setminus \yval} \phi_{z_i}(\U^{(c)})
\end{align*}
Furthermore, observe that $\U^{(c)}$ can be equivalently rewritten in a more compact way:
\begin{align}
\U^{(c)}(S) = \ind \left[ \sum_{j=1}^{\min(K, |S|)} \wtil_{\alpha_{\xval}^{(S, j)}} \ge 0 \right]
\label{eq:util-alter-compact}
\end{align}
where 
$\wtil_i = 
\begin{cases}
    w_i & y_i = \yval \\
    -w_i & y_i = c \\
    0 & \text{otherwise}
\end{cases}
$. 
This formulation (\ref{eq:util-alter-compact}) mirrors the structure of (\ref{eq:util-binary}), differing only in the weight definition $\wtil_i$. This similarity means that Algorithm \ref{alg:efficient-wknn-readable} can be easily adapted to compute the Shapley value $\phi_{z_i}(\U^{(c)})$. Hence, we can first compute $\phi_{z_i}(\U^{(c)})$ for each $c \in [C] \setminus \yval$ individually, and then aggregate these values. While this might imply an inevitable factor of $C$ in the computational complexity, efficiency gains can be made. Specifically, every data point $z_i$ with $y_i \notin \{ \yval, c \}$ has a weight $w_i=0$. Hence it is a null player that yields a Shapley value of $\phi_{z_i}(\U^{(c)}) = 0$. Moreover, a simple result from the literature is that excluding null players does not affect the Shapley values of other players (see Theorem 5 in \cite{wang2023notegroup}). Hence, we can instead compute the Shapley value for a more simplified utility function that is the same as (\ref{eq:util-alter-compact}) but narrow to the subset $D_{\yval, c} \subseteq D$ that comprises only data points labeled $\yval$ or $c$. As a result, the computational time to compute the Shapley value for $\U^{(c)}$ reduces to $O(K |D_{\yval, c}|^2 \nwspace)$. This provides a huge runtime saving when the dataset is balanced. 

\begin{theorem}
For a class-balanced training dataset $D$ with $C$ classes, the time complexity is $\{\phi_{z_i}(\Ualter)\}_{z_i \in D}$ is 
$O\left(\frac{K^2 N^2 \nwspace}{C}\right)$. 
\label{thm:runtime-for-multiclass-heuristic}
\end{theorem}

Remarkably, this methodology is even more efficient than its binary classification counterpart. 

